Size distribution of primary submicron particles and larger aggregates in solvent induced asphaltene precipitation

Asphaltene precipitation is a crucial phase separation phenomenon in the oil industry, especially in paraffinic froth treatment to extract bitumen from oil sands ores. This work reveals the formation of particles at 0.2 to 0.4 um in radius, defined as a primary sub-micron particle (PSMP), which is ubiquitous from diffusive mixing between asphaltene solution and any of 23 types of precipitants examined in our experiments. The yield and quantity of asphaltene particles are affected not only by the Hildebrand solubility parameter of the precipitants but also by the diffusion coefficients of the asphaltene solution and the precipitant. The Population Balance Model (PBM) with the Hildebrand solubility parameter has been used to model particle size distribution. Good agreement has been achieved between numerical predictions and the experimental data. It indicates that the colloid theory can describe the size distribution of PSMP and larger aggregates. Therefore, this study provides new insight into the mechanism for the dependence of yield and size distribution of the precipitated asphaltene particles on the composition of precipitants and adding inhibitors. Controlling of asphaltene yield and size distribution may be applied to the process of hydrocarbon separation or asphaltene precipitation prevention.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
